HRTF upsampling with a generative adversarial network using a gnomonic equiangular projection

An individualised head-related transfer function (HRTF) is very important for creating realistic virtual reality (VR) and augmented reality (AR) environments. However, acoustically measuring high-quality HRTFs requires expensive equipment and an acoustic lab setting. To overcome these limitations and to make this measurement more efficient HRTF upsampling has been exploited in the past where a high-resolution HRTF is created from a low-resolution one. This paper demonstrates how generative adversarial networks (GANs) can be applied to HRTF upsampling. We propose a novel approach that transforms the HRTF data for direct use with a convolutional super-resolution generative adversarial network (SRGAN). This new approach is benchmarked against three baselines: barycentric upsampling, spherical harmonic (SH) upsampling and an HRTF selection approach. Experimental results show that the proposed method outperforms all three baselines in terms of log-spectral distortion (LSD) and localisation performance using perceptual models when the input HRTF is sparse (less than 20 measured positions).

==> gen_images.tex <==
% % \documentclass[journal]{IEEEtran}
% \documentclass[10pt,twocolumn,twoside]{IEEEtran}
% % \documentclass[11pt,draftcls,onecolumn]{IEEEtran}

% \usepackage{lipsum}
% \usepackage{graphicx}
% \usepackage{geometry}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
% \usepackage{cite}
% \ifCLASSOPTIONcompsoc
%     \usepackage[caption=false, font=normalsize, labelfont=sf, textfont=sf]{subfig}
% \else
% \usepackage[caption=false, font=footnotesize]{subfig}
% \fi

% \newcommand{\code}[1]{{\fontfamily{qcr}\selectfont #1}}

% \renewcommand{\algorithmiccomment}[1]{\hfill{\color{black!60}$\triangleright$}\textit{ \color{black!60} #1}}
% \makeatletter
% \renewcommand{\ALG@name}{\small Algorithm}
% \makeatother
% \makeatletter
% \def\BState{\State\hskip-\ALG@thistlm}
% \makeatother

% % *** GRAPHICS RELATED PACKAGES ***
% %
% \ifCLASSINFOpdf
%   % \usepackage[pdftex]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../pdf/}{../jpeg/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% \else
%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%   % will default to the driver specified in the system graphics.cfg if no
%   % driver is specified.
%   % \usepackage[dvips]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../eps/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.eps}
% \fi

% \usepackage{amsmath,graphicx,url}
% \usepackage{tabularx}
% \usepackage{amssymb}
% \usepackage{float}
% \usepackage[nolist,nohyperlinks]{acronym}
% \usepackage{multirow}
% \usepackage{tikz}
% \usepackage[none]{hyphenat}
% \usepackage[flushleft]{threeparttable}
% \usepackage[percent]{overpic}
% \usetikzlibrary{positioning,chains}
% \usetikzlibrary{shapes,arrows}
% \usetikzlibrary{shapes.multipart}
% \usepackage{siunitx}
% \usepackage{tikz-timing}
% \usepackage{pgfplots}
% \newcommand{\matr}[1]{\mathbf{#1}}
% % \usepackage{romannum}
% % \usepackage{flushend}
% \usepackage{balance}
% \renewcommand{\thesubfigure}{(\alph{subfigure})}

% % \usepackage[T2A]{fontenc}
% % \usepackage[utf8]{inputenc}
% % \usepackage[english,russian]{babel}

% % correct bad hyphenation here
% \hyphenation{op-tical net-works semi-conduc-tor}

% \definecolor{c1}{HTML}{33903F}
% \definecolor{c2}{HTML}{C61616}
% \definecolor{c3}{HTML}{0d5593}
% \definecolor{c4}{HTML}{d96459}
% \definecolor{c5}{HTML}{4B4B4B}

% \pgfplotsset{compat=1.14} 

% \begin{document}

% % \eject \pdfpagewidth=3.205in \pdfpageheight=2.175in
% % \newgeometry{margin=-1.15in,top=-10.08in}
% % \input{images/tikz/systems_overview_1}

% % \eject \pdfpagewidth=3.205in \pdfpageheight=2.12in
% % \newgeometry{margin=-1.15in,top=-10.12in}
% % \input{images/tikz/systems_overview_2}

% % \eject \pdfpagewidth=3.303in \pdfpageheight=0.69in
% % \newgeometry{margin=-0.87in,top=-11.22in}
% % \input{images/tikz/evaluation}

% % \eject \pdfpagewidth=3.25in \pdfpageheight=1.32in
% % \newgeometry{margin=-0.92in,top=-10.65in}
% % \input{images/tikz/overlap}

% % \eject \pdfpagewidth=1.765in \pdfpageheight=1.45in
% % \newgeometry{margin=-2.46in,top=-12.05in}
% % \input{images/tikz/mht}

% % \eject \pdfpagewidth=4.26in \pdfpageheight=1.4in
% % \newgeometry{margin=-0.02in,top=-9.65in}
% % \input{images/tikz/track_hypotheses}

% % \eject \pdfpagewidth=3.55in \pdfpageheight=4.02in
% % \newgeometry{margin=-0.62in,top=-7.65in}
% % \input{figures/tikz/mht_flowchart}

% \end{document}

